Galaxy Formation Spanning Cosmic History

Over the past several decades, galaxy formation theory has met with significant successes. In order to test current theories thoroughly we require predictions for as yet unprobed regimes. To this end, we describe a new implementation of the Galform semi-analytic model of galaxy formation. Our motivation is the success of the model described by Bower et al. in explaining many aspects of galaxy formation. Despite this success, the Bower et al. model fails to match some observational constraints and certain aspects of its physical implementation are not as realistic as we would like. The model described in this work includes substantially updated physics, taking into account developments in our understanding over the past decade, and removes certain limiting assumptions made by this (and most other) semi-analytic models. This allows it to be exploited reliably in high-redshift and low mass regimes. Furthermore, we have performed an exhaustive search of model parameter space to find a particular set of model parameters which produce results in good agreement with a wide range of observational data (luminosity functions, galaxy sizes and dynamics, clustering, colours, metal content) over a wide range of redshifts. This model represents a solid basis on which to perform calculations of galaxy formation in as yet unprobed regimes.

==> Data/BestModelsTable.tex <==
{\bf Parameter} &  \multicolumn{2}{c}{\begin{sideways}{\bf Overall}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Star Formation Rate}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf b{\boldmath $_{\rm J}$} \& K LFs}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf 60$\mu$m LF}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf K20 LFs}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Morphological LFs}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf {\boldmath $z=3$} UV LF}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf {\boldmath $z=5$} \& 6 UV LFs}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Colours}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Tully-Fisher}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Sizes}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Metallicity}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\boldmath $M_{\rm Hy}/L_{\rm B}$}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Clustering}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf SMBHs}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Local Group LF}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Local Group Sizes}\end{sideways}} & \multicolumn{2}{c}{\begin{sideways}{\bf Local Group {\boldmath $Z$}'s}\end{sideways}} \\
\hline
\rowcolor[gray]{1.0}[1pt][2pt]
$\Lambda_0$ & \BestFitlambda0 & 0&723 & 0&723 & 0&717 & 0&721 & 0&720 & 0&717 & 0&721 & 0&723 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\Omega_{\rm b}$ & \BestFitomegab & 0&0445 & 0&0465 & 0&0479 & 0&0471 & 0&0491 & 0&0452 & 0&0477 & 0&0482 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$h_0$ & \BestFith0 & 0&677 & 0&711 & 0&714 & 0&707 & 0&726 & 0&700 & 0&703 & 0&689 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\sigma_8$ & \BestFitsigma8 & 0&799 & 0&786 & 0&805 & 0&785 & 0&788 & 0&779 & 0&765 & 0&808 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$n_{\rm s}$ & \BestFitnspec & 0&955 & 0&957 & 0&939 & 0&952 & 0&960 & 0&947 & 0&946 & 0&951 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\alpha_{\rm reheat}$ & \BestFitalphareheat & 2&68 & 1&98 & 1&47 & 1&76 & 2&34 & 2&38 & 2&16 & 2&26 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\alpha_{\rm cool}$ & \BestFitalphacool & {\bf 0}&{\bf 571} & {\bf 2}&{\bf 31} & 1&12 & 1&50 & 2&67 & 2&10 & 2&81 & 0&588 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\alpha_{\rm remove}$ & \BestFitalphaCooledRemove & 0&842 & 0&692 & 0&133 & 0&0986 & 0&547 & 0&0607 & 0&228 & 0&162 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$a_{\rm core}$ & \BestFitcore & 0&128 & 0&168 & 0&155 & 0&0695 & 0&187 & 0&0515 & 0&142 & 0&109 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$A_{\rm ac}$ & \BestFitAGnedin & 0&920 & 0&819 & 0&764 & 0&780 & 0&770 & 0&804 & 0&746 & 0&880 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$w_{\rm ac}$ & \BestFitwGnedin & 0&792 & 0&954 & 0&941 & 0&957 & 0&989 & 0&968 & 0&972 & 0&868 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\epsilon_\star$ & \BestFitepsilonStar & {\bf 0}&{\bf 0695} & 0&0453 & 0&0375 & 0&00520 & 0&0281 & 0&0223 & 0&300 & 0&0153 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\alpha_\star$ & \BestFitalphastar & -2&11 & -2&73 & -2&65 & {\bf -2}&{\bf 05} & -3&43 & -2&95 & -3&68 & {\bf -0}&{\bf 392} \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\epsilon_{\rm d,gas}$ & \BestFitstabledisk & 0&734 & 0&743 & 0&726 & 0&829 & 0&774 & 0&804 & 0&957 & 0&808 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$V_{\rm hot,disk}$ & \BestFitvhotdisk & 425&0 & 532&0 & 421&0 & 491&0 & 411&0 & 506&0 & 546&0 & 459&0 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$V_{\rm hot,burst}$ & \BestFitvhotburst & 130&0 & 470&0 & 413&0 & 539&0 & 498&0 & 544&0 & 488&0 & 242&0 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\alpha_{\rm hot}$ & \BestFitalphahot & 2&61 & 2&81 & 2&73 & {\bf 3}&{\bf 57} & 3&50 & 3&53 & 3&15 & 2&95 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\lambda_{\rm expel,disk}$ & \BestFitlambdaExpelDisk & 0&738 & 0&252 & 0&920 & 0&273 & 0&477 & 0&571 & 0&266 & 0&607 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\lambda_{\rm expel,burst}$ & \BestFitlambdaExpelBurst & 6&49 & 7&90 & 5&39 & 5&23 & 7&46 & 6&62 & 9&23 & 6&55 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\epsilon_{\rm strip}$ & \BestFitRamPressureTransferFraction & 0&951 & 0&696 & 0&248 & 0&207 & 0&0997 & 0&739 & 0&355 & 0&145 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$f_{\rm ellip}$ & \BestFitfellip & 0&184 & 0&0946 & 0&0658 & 0&0250 & {\bf 0}&{\bf 327} & 0&0246 & 0&118 & 0&0250 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$f_{\rm burst}$ & \BestFitfburst & 0&260 & 0&310 & 0&477 & 0&297 & 0&286 & 0&281 & 0&451 & 0&183 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$f_{\rm gas,burst}$ & \BestFitfgasburst & 0&209 & 0&0817 & {\bf 0}&{\bf 0553} & 0&164 & 0&349 & 0&236 & 0&225 & 0&452 \\
\rowcolor[gray]{0.9}[1pt][2pt]
${\rm B/T}_{\rm burst}$ & \BestFitbtburst & 0&538 & 0&889 & 0&890 & 0&517 & 0&367 & 1&00 & 0&215 & 0&928 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\epsilon_\bullet$ & \BestFitepsilonSMBHEddington & 0&0437 & 0&00596 & 0&0363 & 0&00877 & 0&0542 & 0&00423 & 0&0407 & 0&0130 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\eta_\bullet$ & \BestFitetaSMBH & 0&0596 & 0&00476 & 0&00711 & 0&00188 & 0&0137 & 0&00728 & 0&0307 & 0&00788 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$F_\bullet$ & \BestFitFSMBH & 0&00818 & 0&00289 & 0&00628 & 0&0206 & 0&0233 & 0&00190 & 0&0256 & 0&00271 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$V_{\rm cut}$ & \BestFitvcut & 17&0 & 36&5 & 28&4 & 38&7 & 43&9 & 32&9 & 27&7 & 34&5 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$z_{\rm cut}$ & \BestFitzcut & 10&1 & 11&7 & 10&9 & 12&7 & 12&4 & 10&8 & 11&9 & 12&8 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\Lambda_0$ & \BestFitlambda0 & 0&723 & 0&723 & 0&717 & 0&721 & 0&720 & 0&717 & 0&721 & 0&723 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\Omega_{\rm b}$ & \BestFitomegab & 0&0445 & 0&0465 & 0&0479 & 0&0471 & 0&0491 & 0&0452 & 0&0477 & 0&0482 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$h_0$ & \BestFith0 & 0&677 & 0&711 & 0&714 & 0&707 & 0&726 & 0&700 & 0&703 & 0&689 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\sigma_8$ & \BestFitsigma8 & 0&799 & 0&786 & 0&805 & 0&785 & 0&788 & 0&779 & 0&765 & 0&808 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$n_{\rm s}$ & \BestFitnspec & 0&955 & 0&957 & 0&939 & 0&952 & 0&960 & 0&947 & 0&946 & 0&951 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\alpha_{\rm reheat}$ & \BestFitalphareheat & 2&68 & 1&98 & 1&47 & 1&76 & 2&34 & 2&38 & 2&16 & 2&26 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\alpha_{\rm cool}$ & \BestFitalphacool & {\bf 0}&{\bf 571} & {\bf 2}&{\bf 31} & 1&12 & 1&50 & 2&67 & 2&10 & 2&81 & 0&588 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\alpha_{\rm remove}$ & \BestFitalphaCooledRemove & 0&842 & 0&692 & 0&133 & 0&0986 & 0&547 & 0&0607 & 0&228 & 0&162 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$a_{\rm core}$ & \BestFitcore & 0&128 & 0&168 & 0&155 & 0&0695 & 0&187 & 0&0515 & 0&142 & 0&109 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$A_{\rm ac}$ & \BestFitAGnedin & 0&920 & 0&819 & 0&764 & 0&780 & 0&770 & 0&804 & 0&746 & 0&880 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$w_{\rm ac}$ & \BestFitwGnedin & 0&792 & 0&954 & 0&941 & 0&957 & 0&989 & 0&968 & 0&972 & 0&868 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\epsilon_\star$ & \BestFitepsilonStar & {\bf 0}&{\bf 0695} & 0&0453 & 0&0375 & 0&00520 & 0&0281 & 0&0223 & 0&300 & 0&0153 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\alpha_\star$ & \BestFitalphastar & -2&11 & -2&73 & -2&65 & {\bf -2}&{\bf 05} & -3&43 & -2&95 & -3&68 & {\bf -0}&{\bf 392} \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\epsilon_{\rm d,gas}$ & \BestFitstabledisk & 0&734 & 0&743 & 0&726 & 0&829 & 0&774 & 0&804 & 0&957 & 0&808 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$V_{\rm hot,disk}$ & \BestFitvhotdisk & 425&0 & 532&0 & 421&0 & 491&0 & 411&0 & 506&0 & 546&0 & 459&0 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$V_{\rm hot,burst}$ & \BestFitvhotburst & 130&0 & 470&0 & 413&0 & 539&0 & 498&0 & 544&0 & 488&0 & 242&0 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\alpha_{\rm hot}$ & \BestFitalphahot & 2&61 & 2&81 & 2&73 & {\bf 3}&{\bf 57} & 3&50 & 3&53 & 3&15 & 2&95 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\lambda_{\rm expel,disk}$ & \BestFitlambdaExpelDisk & 0&738 & 0&252 & 0&920 & 0&273 & 0&477 & 0&571 & 0&266 & 0&607 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\lambda_{\rm expel,burst}$ & \BestFitlambdaExpelBurst & 6&49 & 7&90 & 5&39 & 5&23 & 7&46 & 6&62 & 9&23 & 6&55 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\epsilon_{\rm strip}$ & \BestFitRamPressureTransferFraction & 0&951 & 0&696 & 0&248 & 0&207 & 0&0997 & 0&739 & 0&355 & 0&145 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$f_{\rm ellip}$ & \BestFitfellip & 0&184 & 0&0946 & 0&0658 & 0&0250 & {\bf 0}&{\bf 327} & 0&0246 & 0&118 & 0&0250 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$f_{\rm burst}$ & \BestFitfburst & 0&260 & 0&310 & 0&477 & 0&297 & 0&286 & 0&281 & 0&451 & 0&183 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$f_{\rm gas,burst}$ & \BestFitfgasburst & 0&209 & 0&0817 & {\bf 0}&{\bf 0553} & 0&164 & 0&349 & 0&236 & 0&225 & 0&452 \\
\rowcolor[gray]{0.9}[1pt][2pt]
${\rm B/T}_{\rm burst}$ & \BestFitbtburst & 0&538 & 0&889 & 0&890 & 0&517 & 0&367 & 1&00 & 0&215 & 0&928 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$\epsilon_\bullet$ & \BestFitepsilonSMBHEddington & 0&0437 & 0&00596 & 0&0363 & 0&00877 & 0&0542 & 0&00423 & 0&0407 & 0&0130 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$\eta_\bullet$ & \BestFitetaSMBH & 0&0596 & 0&00476 & 0&00711 & 0&00188 & 0&0137 & 0&00728 & 0&0307 & 0&00788 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$F_\bullet$ & \BestFitFSMBH & 0&00818 & 0&00289 & 0&00628 & 0&0206 & 0&0233 & 0&00190 & 0&0256 & 0&00271 \\
\rowcolor[gray]{0.9}[1pt][2pt]
$V_{\rm cut}$ & \BestFitvcut & 17&0 & 36&5 & 28&4 & 38&7 & 43&9 & 32&9 & 27&7 & 34&5 \\
\rowcolor[gray]{1.0}[1pt][2pt]
$z_{\rm cut}$ & \BestFitzcut & 10&1 & 11&7 & 10&9 & 12&7 & 12&4 & 10&8 & 11&9 & 12&8 \\
\hline


==> Data/PCA_Table.tex <==
{\bf PCA} & \multicolumn{2}{c}{\boldmath{$\sigma$}} & \multicolumn{2}{c}{\boldmath{$V_{\rm hot,disk}$}} & \multicolumn{2}{c}{\boldmath{$V_{\rm hot,burst}$}} & \multicolumn{2}{c}{\boldmath{$\alpha_{\rm hot}$}} & \multicolumn{2}{c}{\boldmath{$\alpha_{\rm reheat}$}} & \multicolumn{2}{c}{\boldmath{$\alpha_{\rm cool}$}} & \multicolumn{2}{c}{\boldmath{$\alpha_{\rm remove}$}} & \multicolumn{2}{c}{\boldmath{$\epsilon_\star$}} & \multicolumn{2}{c}{\boldmath{$\epsilon_{\rm d,gas}$}} & \multicolumn{2}{c}{\boldmath{$V_{\rm cut}$}} & \multicolumn{2}{c}{\boldmath{$z_{\rm cut}$}} & \multicolumn{2}{c}{\boldmath{$\alpha_\star$}} & \multicolumn{2}{c}{\boldmath{$f_{\rm ellip}$}} & \multicolumn{2}{c}{\boldmath{$f_{\rm burst}$}} & \multicolumn{2}{c}{\boldmath{$F_\bullet$}} & \multicolumn{2}{c}{\boldmath{$a_{\rm core}$}} & \multicolumn{2}{c}{\boldmath{$\epsilon_\bullet$}} & \multicolumn{2}{c}{\boldmath{$\eta_\bullet$}} & \multicolumn{2}{c}{\boldmath{$\lambda_{\rm expel,disk}$}} & \multicolumn{2}{c}{\boldmath{$\lambda_{\rm expel,burst}$}} & \multicolumn{2}{c}{\boldmath{$h_0$}} & \multicolumn{2}{c}{\boldmath{$\Omega_{\rm b}$}} & \multicolumn{2}{c}{\boldmath{$\Lambda_0$}} & \multicolumn{2}{c}{\boldmath{$\sigma_8$}} & \multicolumn{2}{c}{\boldmath{$n_{\rm s}$}} & \multicolumn{2}{c}{\boldmath{$\epsilon_{\rm strip}$}} & \multicolumn{2}{c}{\boldmath{$f_{\rm gas,burst}$}} & \multicolumn{2}{c}{\boldmath{$A_{\rm ac}$}} & \multicolumn{2}{c}{\boldmath{$w_{\rm ac}$}} & \multicolumn{2}{c}{\boldmath{$B/T_{\rm burst}$}} \\
\hline
PCA 1 &  0&025 & -0&097 & -0&051 & {\bf -0}&{\bf 379} &  0&297 &  0&045 & -0&227 & -0&261 &  0&249 &  0&022 & {\bf -0}&{\bf 352} & {\bf  0}&{\bf 425} & -0&288 &  0&187 & -0&168 & -0&123 & -0&162 &  0&033 &  0&093 &  0&047 &  0&186 & -0&049 &  0&027 & -0&168 &  0&036 & -0&003 & -0&024 &  0&009 & -0&016 &  0&006 \\
PCA 2 &  0&043 & -0&143 &  0&097 &  0&008 &  0&109 &  0&152 &  0&050 & -0&111 &  0&092 & -0&032 &  0&182 &  0&011 &  0&145 &  0&048 &  0&073 &  0&095 & -0&053 & -0&059 &  0&093 & {\bf -0}&{\bf 486} &  0&115 & {\bf -0}&{\bf 627} & -0&283 & -0&040 & -0&283 & -0&054 &  0&025 & -0&052 &  0&052 & -0&105 \\
PCA 3 &  0&045 & {\bf  0}&{\bf 420} & -0&213 & -0&027 &  0&138 &  0&147 &  0&093 & -0&010 &  0&194 & {\bf  0}&{\bf 364} & -0&039 &  0&166 &  0&208 &  0&297 &  0&285 & -0&029 & {\bf  0}&{\bf 395} &  0&049 &  0&199 &  0&006 & -0&185 & -0&116 &  0&086 &  0&203 &  0&122 &  0&007 &  0&054 & -0&033 & -0&020 &  0&037 \\
PCA 4 &  0&051 &  0&030 & -0&023 & -0&284 & {\bf -0}&{\bf 405} & -0&011 & {\bf  0}&{\bf 410} & {\bf -0}&{\bf 424} & -0&117 & -0&055 & -0&056 & {\bf  0}&{\bf 392} &  0&060 & -0&233 &  0&230 &  0&047 &  0&006 & -0&073 & -0&296 & -0&021 & -0&138 &  0&004 & -0&032 & -0&032 &  0&008 & -0&057 &  0&019 & -0&027 &  0&010 & -0&008 \\
PCA 5 &  0&064 &  0&203 &  0&107 & -0&270 & -0&173 &  0&014 & -0&050 &  0&046 &  0&135 & -0&076 &  0&174 & -0&230 & -0&158 &  0&258 &  0&147 & -0&102 & -0&128 & {\bf  0}&{\bf 639} & -0&234 & -0&234 & -0&066 &  0&058 & -0&128 & -0&140 &  0&158 &  0&046 & -0&045 &  0&033 &  0&012 & -0&008 \\
PCA 6 &  0&083 &  0&216 &  0&053 & -0&060 &  0&072 &  0&112 & -0&159 & -0&129 & -0&200 &  0&217 & -0&081 & -0&092 & -0&142 & {\bf -0}&{\bf 629} & -0&265 & -0&260 &  0&231 &  0&209 &  0&050 & -0&241 &  0&045 & -0&117 &  0&031 &  0&135 &  0&141 & -0&117 & -0&018 & -0&065 & -0&025 & -0&011 \\
PCA 7 &  0&104 &  0&056 & -0&023 & -0&152 & -0&024 & -0&008 &  0&019 &  0&112 & -0&071 &  0&121 & -0&027 & -0&103 & -0&088 & -0&102 &  0&057 & -0&004 & -0&116 & -0&001 &  0&102 & {\bf  0}&{\bf 575} & -0&070 & -0&290 & {\bf -0}&{\bf 658} &  0&033 &  0&149 & -0&074 & -0&049 & -0&006 &  0&013 & -0&007 \\
PCA 8 &  0&106 &  0&108 &  0&271 & {\bf  0}&{\bf 471} &  0&029 & {\bf -0}&{\bf 616} &  0&028 & -0&205 &  0&289 &  0&145 & -0&225 &  0&040 & -0&068 & -0&043 &  0&115 & -0&149 & -0&157 &  0&066 & -0&053 & -0&044 & -0&137 & -0&109 & -0&059 &  0&041 &  0&009 & -0&046 & -0&001 &  0&008 &  0&002 & -0&001 \\
PCA 9 &  0&111 & -0&288 & {\bf  0}&{\bf 423} & -0&038 & -0&219 &  0&255 &  0&064 &  0&299 &  0&311 & {\bf  0}&{\bf 579} &  0&027 &  0&138 & -0&070 & -0&109 &  0&049 &  0&066 & -0&030 &  0&000 & -0&080 &  0&015 &  0&123 &  0&132 &  0&032 &  0&070 & -0&058 & -0&016 &  0&009 &  0&063 & -0&022 & -0&026 \\
PCA 10 &  0&114 & -0&296 & -0&212 & {\bf  0}&{\bf 407} &  0&319 & {\bf  0}&{\bf 411} &  0&222 & -0&236 & -0&131 &  0&089 & -0&152 & -0&116 & -0&237 & -0&018 &  0&287 & -0&032 & -0&051 &  0&267 & -0&154 &  0&074 & -0&054 &  0&098 & -0&050 & -0&047 & -0&053 &  0&008 &  0&007 & -0&006 & -0&024 & -0&021 \\
PCA 11 &  0&122 & -0&029 &  0&041 &  0&007 &  0&001 &  0&000 &  0&013 &  0&008 &  0&040 & -0&043 &  0&047 &  0&004 & -0&002 &  0&033 &  0&010 &  0&049 & -0&006 & -0&022 & -0&007 & -0&019 & -0&015 & -0&001 & -0&012 &  0&003 &  0&025 & -0&085 & -0&308 & {\bf -0}&{\bf 453} & {\bf -0}&{\bf 817} &  0&108 \\
PCA 12 &  0&128 &  0&034 & -0&012 & -0&001 & -0&012 & -0&010 &  0&018 &  0&069 &  0&003 &  0&037 & -0&006 &  0&000 & -0&038 &  0&025 &  0&043 & -0&122 &  0&064 & -0&005 & -0&066 &  0&010 &  0&092 &  0&043 & -0&037 & -0&072 & -0&263 & -0&139 & -0&252 & {\bf -0}&{\bf 411} & {\bf  0}&{\bf 409} & {\bf  0}&{\bf 678} \\
PCA 13 &  0&137 & -0&050 & {\bf -0}&{\bf 503} &  0&047 & -0&140 & -0&118 & -0&177 & -0&020 &  0&166 &  0&258 &  0&056 & -0&124 & -0&219 &  0&092 & -0&252 &  0&200 &  0&107 & -0&171 & {\bf -0}&{\bf 560} & -0&061 &  0&002 & -0&178 & -0&027 &  0&098 &  0&018 & -0&045 & -0&009 &  0&036 & -0&016 & -0&001 \\
PCA 14 &  0&142 & -0&022 & {\bf -0}&{\bf 482} &  0&032 & -0&179 & -0&032 & {\bf  0}&{\bf 467} &  0&195 &  0&317 & -0&022 & -0&017 & -0&015 &  0&019 & -0&178 & -0&192 & -0&158 & {\bf -0}&{\bf 335} &  0&153 &  0&327 & -0&087 &  0&128 & -0&031 &  0&077 &  0&063 &  0&035 &  0&043 & -0&037 &  0&003 & -0&011 &  0&027 \\
PCA 15 &  0&147 &  0&015 & -0&007 & -0&033 & -0&194 &  0&101 & -0&105 &  0&151 &  0&252 & -0&307 & {\bf -0}&{\bf 680} & -0&224 &  0&067 & -0&149 &  0&205 &  0&256 &  0&255 &  0&034 & -0&012 & -0&062 &  0&112 & -0&036 & -0&059 &  0&038 & -0&074 &  0&025 & -0&112 &  0&047 &  0&003 & -0&039 \\
PCA 16 &  0&155 & -0&135 & -0&287 &  0&101 & -0&250 & -0&162 & {\bf -0}&{\bf 505} & -0&079 & -0&157 &  0&139 &  0&140 &  0&231 &  0&124 & -0&140 & {\bf  0}&{\bf 352} &  0&194 & -0&109 &  0&303 &  0&237 &  0&043 &  0&223 &  0&021 &  0&037 &  0&016 & -0&091 & -0&025 & -0&022 &  0&022 & -0&029 &  0&025 \\
PCA 17 &  0&157 & -0&076 & -0&030 & -0&017 &  0&042 & -0&003 &  0&014 &  0&096 &  0&049 & -0&110 &  0&011 &  0&011 & -0&011 &  0&058 &  0&032 &  0&039 & -0&004 &  0&024 &  0&047 & -0&044 & -0&089 &  0&080 &  0&040 &  0&014 &  0&075 & {\bf -0}&{\bf 950} &  0&112 &  0&134 & -0&001 & -0&024 \\
PCA 18 &  0&168 &  0&147 &  0&080 & {\bf  0}&{\bf 474} & {\bf -0}&{\bf 435} &  0&302 & -0&074 &  0&061 & -0&085 & -0&216 & -0&025 & {\bf  0}&{\bf 384} & -0&202 &  0&236 & -0&279 & -0&131 &  0&134 &  0&068 &  0&055 &  0&030 &  0&030 & -0&122 & -0&123 & -0&013 &  0&068 & -0&018 & -0&011 &  0&038 & -0&007 &  0&007 \\
PCA 19 &  0&174 &  0&143 &  0&106 &  0&007 &  0&049 & -0&191 &  0&313 & -0&075 & -0&143 &  0&000 &  0&093 & -0&074 & -0&322 &  0&124 &  0&124 &  0&204 &  0&189 & -0&023 &  0&051 &  0&023 & {\bf  0}&{\bf 727} & -0&017 &  0&029 &  0&123 &  0&160 & -0&042 &  0&024 &  0&050 & -0&019 &  0&007 \\
PCA 20 &  0&182 & -0&063 &  0&135 & -0&109 & -0&203 &  0&094 & -0&033 & -0&117 & -0&118 & -0&014 & -0&077 & -0&237 & -0&140 &  0&147 &  0&057 & -0&075 & -0&219 &  0&046 &  0&041 &  0&269 & -0&099 & {\bf -0}&{\bf 458} & {\bf  0}&{\bf 551} & {\bf  0}&{\bf 334} & -0&087 & -0&047 & -0&049 & -0&047 &  0&034 &  0&005 \\
PCA 21 &  0&189 & -0&178 & -0&011 & -0&064 & {\bf -0}&{\bf 335} & -0&050 &  0&032 & {\bf -0}&{\bf 375} & -0&127 &  0&290 & -0&146 & {\bf -0}&{\bf 360} & -0&089 &  0&269 & -0&161 &  0&032 &  0&116 & -0&116 & {\bf  0}&{\bf 430} & -0&168 & -0&131 &  0&204 & -0&150 & -0&162 & -0&023 & -0&029 & -0&010 & -0&022 &  0&005 &  0&001 \\
PCA 22 &  0&196 &  0&009 &  0&002 &  0&085 & -0&031 & -0&016 &  0&062 &  0&134 & -0&048 &  0&130 & -0&047 & -0&040 &  0&038 & -0&093 &  0&034 &  0&150 &  0&058 &  0&001 &  0&010 &  0&082 & -0&017 & -0&322 &  0&291 & {\bf -0}&{\bf 773} &  0&318 & -0&012 &  0&085 & -0&072 &  0&013 &  0&058 \\
PCA 23 &  0&204 & -0&068 & -0&066 & -0&028 & -0&062 &  0&005 & -0&107 & -0&008 &  0&306 & -0&195 & {\bf  0}&{\bf 339} & -0&044 & {\bf -0}&{\bf 484} & -0&190 & {\bf  0}&{\bf 357} & -0&246 &  0&245 & -0&293 &  0&183 &  0&006 & -0&152 &  0&001 &  0&058 & -0&110 & -0&015 &  0&051 & -0&174 &  0&109 &  0&020 & -0&071 \\
PCA 24 &  0&231 & {\bf  0}&{\bf 431} &  0&074 &  0&132 & -0&025 & {\bf  0}&{\bf 346} & -0&148 & {\bf -0}&{\bf 374} & {\bf  0}&{\bf 338} & -0&033 &  0&157 & -0&176 &  0&055 & -0&146 & -0&035 &  0&292 & {\bf -0}&{\bf 348} & -0&174 &  0&032 &  0&104 &  0&099 &  0&151 &  0&011 & -0&043 &  0&053 & -0&057 &  0&105 & -0&072 &  0&042 &  0&077 \\
PCA 25 &  0&242 & -0&266 &  0&025 & -0&027 & -0&025 & -0&022 & -0&068 &  0&041 &  0&074 & -0&154 & -0&005 &  0&022 & -0&144 & -0&036 &  0&073 &  0&091 &  0&020 & -0&014 &  0&074 & -0&126 & -0&122 & -0&032 & -0&067 &  0&232 & {\bf  0}&{\bf 359} &  0&127 & {\bf  0}&{\bf 657} & -0&280 & -0&020 &  0&322 \\
PCA 26 &  0&279 & -0&077 & -0&005 &  0&042 &  0&021 & -0&015 & -0&018 &  0&051 &  0&002 & -0&011 &  0&007 &  0&086 & -0&041 &  0&034 &  0&009 &  0&154 & -0&052 & -0&015 &  0&030 & -0&066 & -0&049 &  0&084 &  0&018 &  0&111 &  0&314 & -0&034 & -0&270 & {\bf -0}&{\bf 577} & {\bf  0}&{\bf 384} & {\bf -0}&{\bf 521} \\
PCA 27 &  0&343 & -0&183 &  0&009 &  0&054 & -0&017 &  0&111 & -0&097 & -0&082 & -0&044 &  0&005 & -0&042 & -0&051 &  0&281 &  0&070 &  0&139 & -0&233 & -0&158 & -0&232 & -0&083 & -0&179 &  0&131 & -0&042 & -0&041 &  0&120 & {\bf  0}&{\bf 596} &  0&016 & {\bf -0}&{\bf 359} &  0&277 &  0&031 &  0&236 \\
PCA 28 &  0&366 & {\bf -0}&{\bf 333} &  0&069 &  0&023 &  0&003 & -0&039 &  0&040 & -0&326 & {\bf  0}&{\bf 350} & -0&151 &  0&227 & -0&063 &  0&329 & -0&031 & -0&249 & -0&047 & {\bf  0}&{\bf 414} &  0&301 & -0&025 & {\bf  0}&{\bf 335} &  0&111 & -0&046 &  0&031 &  0&011 &  0&071 & -0&013 & -0&042 & -0&025 &  0&053 & -0&006 \\
PCA 29 &  0&436 & -0&038 &  0&092 & -0&004 &  0&158 & -0&047 &  0&109 & -0&009 & -0&020 & -0&041 &  0&081 &  0&155 & -0&200 & -0&085 & -0&176 & {\bf  0}&{\bf 598} &  0&017 &  0&176 &  0&173 & -0&080 & {\bf -0}&{\bf 345} & -0&051 &  0&034 &  0&125 &  0&098 &  0&077 & {\bf -0}&{\bf 344} &  0&270 &  0&055 &  0&257 \\
\hline

